NVBleed: Covert and Side-Channel Attacks on NVIDIA Multi-GPU Interconnect

Multi-GPU systems are becoming increasingly important in highperformance computing (HPC) and cloud infrastructure, providing acceleration for data-intensive applications, including machine learning workloads. These systems consist of multiple GPUs interconnected through high-speed networking links such as NVIDIA's NVLink. In this work, we explore whether the interconnect on such systems can offer a novel source of leakage, enabling new forms of covert and side-channel attacks. Specifically, we reverse engineer the operations of NVlink and identify two primary sources of leakage: timing variations due to contention and accessible performance counters that disclose communication patterns. The leakage is visible remotely and even across VM instances in the cloud, enabling potentially dangerous attacks. Building on these observations, we develop two types of covert-channel attacks across two GPUs, achieving a bandwidth of over 70 Kbps with an error rate of 4.78% for the contention channel. We develop two end-to-end crossGPU side-channel attacks: application fingerprinting (including 18 high-performance computing and deep learning applications) and 3D graphics character identification within Blender, a multi-GPU rendering application. These attacks are highly effective, achieving F1 scores of up to 97.78% and 91.56%, respectively. We also discover that leakage surprisingly occurs across Virtual Machines on the Google Cloud Platform (GCP) and demonstrate a side-channel attack on Blender, achieving F1 scores exceeding 88%. We also explore potential defenses such as managing access to counters and reducing the resolution of the clock to mitigate the two sources of leakage.

==> arxiv_mode_extraction.tex <==
\subsection{Model Extraction Attack}
In this section, we present an attack methodology aimed at recovering the structure of DNN models when model parallelism is employed during training. This attack capitalizes on the information leakage that occurs through inter-GPU data transaction traces. The primary objective of our attack is to significantly narrow down the search space of potential target DNN architectures. We begin by elucidating the process of correlating DNN model structural secrets with NVLink transaction patterns. Subsequently, we provide a comprehensive overview of our attack procedure. Finally, we present the evaluation results of our study.


\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth]{figures/DNN_recovery_overview.png}
    \vspace{-2.0em}
    \caption{DNN Model extraction overview. 
    }
    \label{fig:two_attacks}
\end{figure*}

\subsubsection{Mapping DNN to NVLink Transaction}
\label{subsec:map_dnn}

DNNs constitute a family of methodologies that transform input into output through a series of repetitive processing units, each known as a \textit{layer}. Our analysis initially focuses on the output sizes of the three most commonly utilized types of layers: Fully-Connected (FC), Convolutional (Conv), and Pooling layers. Alongside these layers, we also analyze their associated hyper-parameters, which are detailed in Table~\ref{tab:hp}. 

The formulas for calculating the output sizes of various layers are provided from Equation~\ref{fc_out} to \ref{pooling_out}. In scenarios where the victim employs model parallelism for DNN training, the layers are distributed across different GPUs. The output feature maps, generated by previous layer, are transmitted to the subsequent layer via the GPU interconnect. An attacker, by analyzing this traffic pattern, can deduce the output size of each layer. Utilizing these equations, it becomes feasible to infer the specific parameters associated with each layer. For instance, the parameter of a Fully Connected (FC) layer, denoted as $N_{i}$, can be directly calculated using Equation~\ref{fc_out}, provided the attacker knows the $Output_{FC}$ and $BatchSize$. 



Additionally, Equation~\ref{contraint1} introduces a constraint regarding hyper-parameters, which plays a pivotal role in result correction as elaborated in Section~\ref{subsec:}.

\begin{table}[ht]
\centering
\caption{Hyper-parameters of DNN layers}
\label{tab:hp}
 \begin{tabular}{C{1cm}|C{1.4cm}|L{4cm}|}
% \hline
\cline{2-3}
           & \textbf{Layer parameter} & \textbf{Definition}                            \\ \hline \hline
\multicolumn{1}{|c|}{FC layer}                       & $N_{i}$                            & Number of neurons of $layer_{i} $                \\ \hline

\multicolumn{1}{|c|}{\multirow{5}{*}{Conv layer} }   & $W_{i}$                           & Width of output feature map of $layer_{i} $             \\ \cline{2-3} 
                    \multicolumn{1}{|c|}{}           & $F$                              & Size of filter                             \\ \cline{2-3} 
                              \multicolumn{1}{|c|}{}   & $C_{i}$                            & Channels of output feature map (Number of filters) \\ \cline{2-3} 
                              \multicolumn{1}{|c|}{}   & $S$                               & Size of stride size                                        \\ \cline{2-3}
                               \multicolumn{1}{|c|}{}   & $P$                               & Size of padding                                        \\ \hline
 \multicolumn{1}{|c|}{\multirow{4}{*}{Pooling layer}} & $W_{i}$                           & Width of output feature map of $layer_{i} $            \\ \cline{2-3} 
                            \multicolumn{1}{|c|}{}     & $F$                              & Size of filter                             \\ \cline{2-3} 
                            \multicolumn{1}{|c|}{}     & $S$                               & Size of stride  \\ \cline{2-3}  
                             \multicolumn{1}{|c|}{}   & $P$                               & Size of padding   
                             \\ \hline
\end{tabular}
\end{table}

\begin{equation}\label{fc_out}
    Output_{FC} 
    = N_{i} \times BatchSize 
\end{equation}
\begin{equation} \label{conv_out}
    Output_{CONV}  
    = {W_{i}}^2 \times C_{i-1} \times BatchSize    
\end{equation}
\begin{equation} \label{pooling_out}
    Output_{pooling}  
    = {W_{pooling}}^2 \times C_{i-1} \times BatchSize    
\end{equation}
\begin{equation} \label{outputsize}
     W_i = \frac{W_{i-1} - F + 2 \times P}{S} +1
\end{equation}
 \begin{equation}\label{pooling}
    W_{pooling} = \frac{W_{i-1} - F}{S} +1
\end{equation}
\begin{equation}\label{contraint1}
    S \le  F \le \frac{W_{i-1}}{2}
\end{equation}

\begin{equation}\label{contraint2}
    P \le  F \le \frac{W_{i-1}}{2}
\end{equation}

\subsubsection{Methodology}


\subsubsection{Evaluation}


\begin{table}
\small
\centering
\begin{tabular}{c|ccc||ccc|}
\cline{2-7}
\multirow{2}{*}{}         & \multicolumn{3}{c||}{\textbf{DGX}}                                                  & \multicolumn{3}{c|}{\textbf{GCP}}                                                   \\ \cline{2-7} 
                          & \multicolumn{1}{c|}{\textbf{F1}}   & \multicolumn{1}{c|}{\textbf{Prec}} & \textbf{Rec}  & \multicolumn{1}{c|}{\textbf{F1}}   & \multicolumn{1}{c|}{\textbf{Prec}} & \textbf{Rec}  \\ \hline \hline
\multicolumn{1}{|c|}{KNN} & \multicolumn{1}{c|}{}          & \multicolumn{1}{c|}{}          &           & \multicolumn{1}{c|}{}          & \multicolumn{1}{c|}{}          &           \\ \hline
\multicolumn{1}{|c|}{DT}  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{}          & \multicolumn{1}{c|}{}          &            \\ \hline

\multicolumn{1}{|c|}{LightGBM} & \multicolumn{1}{c|}{}          & \multicolumn{1}{c|}{}          &         & \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{} & \\ \hline

\end{tabular}
\caption{Iteration segmenter performance: F1 (\%), Precision (\%), and Recall (\%) on DGX and GCP.}
\label{tb:iteration_seg}
\end{table}





\begin{table}
\small
\centering
\begin{tabular}{L{0.1cm}|ccc||ccc|}
\cline{2-7}
\multirow{2}{*}{}         & \multicolumn{3}{c||}{\textbf{DGX}}                                                  & \multicolumn{3}{c|}{\textbf{GCP}}                                                   \\ \cline{2-7} 
                          & \multicolumn{1}{c|}{\textbf{F1}}   & \multicolumn{1}{c|}{\textbf{Prec}} & \textbf{Rec}  & \multicolumn{1}{c|}{\textbf{F1}}   & \multicolumn{1}{c|}{\textbf{Prec}} & \textbf{Rec}  \\ \hline \hline
\multicolumn{1}{|c|}{KNN} & \multicolumn{1}{c|}{}         & \multicolumn{1}{c|}{}          &         & \multicolumn{1}{c|}{\textbf{100.0\%}}          & \multicolumn{1}{c|}{100.0\%}          &   100.0\%          \\ \hline
\multicolumn{1}{|c|}{XGBoost}  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{95.0\%}          & \multicolumn{1}{c|}{94.9\%}          &     94.9\%       \\ \hline

\multicolumn{1}{|c|}{LightGBM} & \multicolumn{1}{c|}{\textbf{}}          & \multicolumn{1}{c|}{}          &       & \multicolumn{1}{c|}{\textbf{100.0\%}}& \multicolumn{1}{c|}{100.0\%} & 100.0\%   \\ \hline

\end{tabular}
\caption{Layer type performance: F1 (\%), Precision (\%), and Recall (\%) on DGX and GCP.}
\label{tb:layer_type}
\end{table}



\begin{table}[]
\centering
\begin{tabular}{c|c||r|}
\cline{2-3}
\textbf{}                      & \textbf{DGX} & \multicolumn{1}{l|}{\textbf{GCP}} \\ \hline \hline
\multicolumn{1}{|l|}{KNN}      &              & 0.9991                            \\ \hline
\multicolumn{1}{|l|}{XGBoost}  &              & 0.9879                            \\ \hline
\multicolumn{1}{|l|}{LightGBM} &              & 0.9934                            \\ \hline
\end{tabular}
\caption{Input size regressor performance: $R^2$ on DGX and GCP.}
\label{tb:input_size}
\end{table}


\begin{table}[]
\centering
\begin{tabular}{c|c||r|}
\cline{2-3}
\textbf{}                      & \textbf{DGX} & \multicolumn{1}{l|}{\textbf{GCP}} \\ \hline \hline
\multicolumn{1}{|l|}{KNN}      &              & 0.9997                            \\ \hline
\multicolumn{1}{|l|}{XGBoost}  &              & 0.7828                            \\ \hline
\multicolumn{1}{|l|}{LightGBM} &              & 0.9840                            \\ \hline
\end{tabular}
\caption{NVLink transfer size regressor performance: $R^2$ on DGX and GCP.}
\label{tb:nvlink_size}
\end{table}

